Smishing Dataset I: Phishing SMS Dataset from Smishtank.com

While smishing (SMS Phishing) attacks have risen to become one of the most common types of social engineering attacks, there is a lack of relevant smishing datasets. One of the biggest challenges in the domain of smishing prevention is the availability of fresh smishing datasets. Additionally, as time persists, smishing campaigns are shut down and the crucial information related to the attack are lost. With the changing nature of smishing attacks, a consistent flow of new smishing examples is needed by both researchers and engineers to create effective defenses. In this paper, we present the community-sourced smishing datasets from the smishtank.com. It provides a wealth of information relevant to combating smishing attacks through the breakdown and analysis of smishing samples at the point of submission. In the contribution of our work, we provide a corpus of 1090 smishing samples that have been publicly submitted through the site. Each message includes information relating to the sender, message body, and any brands referenced in the message. Additionally, when a URL is found, we provide additional information on the domain, VirusTotal results, and a characterization of the URL. Through the open access of fresh smishing data, we empower academia and industries to create robust defenses against this evolving threat.

==> messagestatusreport.tex <==
\paragraph{VirusTotal and Domain History}
\begin{table}[h]
\scriptsize
\centering
\vspace{-5mm}
\begin{tabular}{@{}llllllll@{}}
\toprule
Type & \#N & VT\textgreater{}1 & VT\textgreater{}5 & VT\textgreater{}10 & VT-M & VT-MW & VT-P \\ \midrule
URLS(ALL) & 46 & 43.48\% & 15.22\% & 8.70\% & 28.26\% & 19.57\% & 26.09\% \\
Domains(ALL) & 44 & 25.00\% & 11.36\% & 9.09\% & 20.45\% & 6.82\% & 20.45\% \\ \midrule
URLS(Selected) & 18 & 72.22\% & 11.11\% & 11.11\% & 50.00\% & 22.22\% & 38.89\% \\
Domains(Selected) & 17 & 29.41\% & 5.88\% & 5.88\% & 23.53\% & 11.76\% & 23.53\% \\ \bottomrule
\end{tabular}
\caption{Virus Total reports for all smishing messages and the messages randomly selected for the experiment. }
\label{tab:virus-totals}
\vspace{-3mm}
\end{table}
 In order to better understand what kind of threat these messages posed, we analyzed them through VirusTotal~\cite{virustotal}. The analysis was performed 7 months after the initial experiment, giving time for messages to be reported and find their way onto vendor blacklists. VirusTotal collaborates with over 70 vendors to provide detailed results from scanning files, URLs and domains. Using this service, we looked at the status and domain update timeline for the messages set. In table~\ref{tab:virus-totals} we note the status of the URLs and their domains, as well as the subsequent number of vendors that rated the URLs as malicious. Interestingly, even after 7 months, only a fraction of messages that were identified as malicious were labeled by more than 5 vendors. We also observed that the status of messages changed through redirects and shorteners. By analyzing the final URL instead of original URL, the status of 6 of our redirected URLs changed from malicious to clean. Potentially, the malicious sender could reuse many of their vendor blacklisted URLs by just applying a new URL shortener or redirection path. Additionally, among the messages marked as clean by vendors, we were able to find examples~\cite{onlinethreatalerts} of online communities that discussed those messages as scams. 

Next, we look at the Domain history of the websites referenced in our smishing messages. In terms of creation time, we can positively confirm that (30/46) of the domains were created within 1-3 months of us receiving the messages. When considering last update time, that number jumps to (36/46). The domain timeline of (3/46) messages could not be confirmed due to their unavailability. Another (5/46) messages utilized authentic domains to deliver their smishing messages, so their older creation date is unsurprising. These messages used either private groups on social media sites, or web API to begin phone calls. Next, we witnessed 2 older domains (20+ years old) that were being used to host malicious sites. Surprisingly, when we investigated the domain owner we found that they had been involved in civil suits before for hosting malicious content~\cite{vitalworks}. Finally, out of the 46 collected URLs, only one has been updated since our experiment. 

